Heat Transfer in Gold Interfaces Capped with Thiolated Polyethylene Glycol: A Molecular Dynamics Study

Reverse non-equilibrium molecular dynamics (RNEMD) simulations were used to study heat transport in solvated gold interfaces which have been functionalized with a low molecular weight thiolated polyethylene glycol (PEG). The gold interfaces studied included (111), (110), and (100) facets, as well as spherical nanoparticles with radii of 10 and 20 {\AA}. The embedded atom model (EAM) and the polarizable density-readjusted embedded atom model (DR-EAM) were implemented to determine the effect of metal polarizability on heat transport properties. We find that the interfacial thermal conductance values for thiolated PEG capped interfaces are higher than those for pristine gold interfaces. Hydrogen bonding between the thiolated PEG and solvent differs between planar facets and the nanospheres, suggesting one mechanism for enhanced transfer of energy, while the covalent gold sulfur bond appears to create the largest barrier to thermal conduction. Through analysis of vibrational power spectra, we find an enhanced population at low frequency heat carrying modes for the nanospheres, which may also explain the higher mean G value.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
